Detection Thresholds for the $\beta$-Model on Sparse Graphs

In this paper we study sharp thresholds for detecting sparse signals in $\beta$-models for potentially sparse random graphs. The results demonstrate interesting interplay between graph sparsity, signal sparsity, and signal strength. In regimes of moderately dense signals, irrespective of graph sparsity, the detection thresholds mirror corresponding results in independent Gaussian sequence problems. For sparser signals, extreme graph sparsity implies that all tests are asymptotically powerless, irrespective of the signal strength. On the other hand, sharp detection thresholds are obtained, up to matching constants, on denser graphs. The phase transition mentioned above are sharp. As a crucial ingredient, we study a version of the Higher Criticism Test which is provably sharp up to optimal constants in the regime of sparse signals. The theoretical results are further verified by numerical simulations.

==> binary_macro.tex <==
\catcode`\@=11 % allows @ to be used in control sequences in this format file

\startlocaldefs
\numberwithin{equation}{section}
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\endlocaldefs
%THEOREM Environments ------------------------------------
%\newtheorem{thm}{Theorem}[section]
%\newtheorem{cor}[thm]{Corollary}
\newtheorem{theorem}[thm]{Theorem}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{ass}[thm]{Assumption}
\newtheorem{pri}[thm]{Prior}
%\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
%\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{cor}[thm]{Corollary}
%\numberwithin{equation}{subsection}
\newtheorem{lem}[thm]{Lemma}
%\newtheorem{prop}[thm]{Proposition}
%\newtheorem{ass}[thm]{Assumption}
%\newtheorem{pri}[thm]{Prior}
%\theoremstyle{definition}
%\newtheorem{defn}[thm]{Definition}
\theoremstyle{remark}
\newtheorem{rem}[thm]{Remark}
%\newtheorem{cor}[thm]{Corollary}
%\numberwithin{equation}{subsection}
%% MATH ----------------------------------------------------

%Beta Model Macro: Rajarshi

\def \Pbeta {\mathbb{P}_{\boldsymbol{\beta},\lambda}}
\def \Pzero {\mathbb{P}_{\boldsymbol{\beta}=\mathbf{0},\lambda}}
\def \Ebeta {\mathbb{E}_{\boldsymbol{\beta},\lambda}}
\def \Ezero {\mathbb{E}_{\boldsymbol{\beta}=\mathbf{0},\lambda}}
\def \phibar{\bar{\Phi}}
\def \Vzero {\mathrm{Var}_{\boldsymbol{\beta}=\mathbf{0},\lambda}}


\def \bbeta{\boldsymbol{\beta}}
\def \bx{\mathbf{x}}
%\def \bx{\mathbf{y}}
\def \bX{\mathbf{X}}
\def \risk{\mathrm{Risk}}
\def \alt{\Theta^A_k}
\def \altbino{\Xi^{\Delta}_k}
\def \be{\begin{equs}}
	\def \ee{\end{equs}}
\def \tcr{\textcolor{red}}
\def \tcv{\textcolor{black}}
\def \tcg{\textcolor{black}}
\def \tcbr{\textcolor{black}}
\def\wa {\mathrm{WA}(n^*,n_*,r^*,r_*,Q,\gamma)}
\def\sa{\mathrm{ANOVA}(r)}
\def \tglrt{\mathsf{T}_\mathrm{GLRT}}
\def \tglrtnew{\mathsf{T}_\mathrm{GLRT}}
%\def \tglrt{\mathsf{T}_\mathrm{GLRT}}
\def \thc{\mathsf{T}_\mathrm{HC}}
\def \thcnew{\mathsf{T}_\mathrm{HC}}
\def \I{\mathcal{I}}
\def \bdelta {\mathbf{\delta}}
\def \bnu {\mathbf{\nu}}
\def \thetap {\theta^{'}(0)}
\def \E{\mathbb{E}}
\def \P{\mathbb{P}}
\def \hpleft {Z_1 <\frac{r}{2}-\sqrt{2\log{p}}\sqrt{\frac{r}{4}}}
\def \hpright {Z_1 >\frac{r}{2}+\sqrt{2\log{p}}\sqrt{\frac{r}{4}}}
\def \hplefto {Z_1 \geq \frac{r}{2}-\sqrt{2\log{p}}\sqrt{\frac{r}{4}}}
\def \hprighto {Z_1 \leq \frac{r}{2}+\sqrt{2\log{p}}\sqrt{\frac{r}{4}}}
\def \hpj {Z_j \in H_p}
\def \tp {\sqrt{2\log{p}}}
\def \lp {\log{p}}
%\def \thetap{\theta'(0)}
\def \astar {A^{*}}
\def \errorx {(\log{r}+x)}
\def \sqr{\sqrt{r}}
\def \xionej{\xi_1^j}
\def \xitwoj{\xi_2^j}
\def \thetaf {\frac{\theta(A)}{\theta(-A)}}
\def \thetapl{\theta(A)}
\def \thetam{\theta(-A)}
\def \zj{Z_j}
\def \BC{\mathrm{BC}}
\def \fhat{\hat{f}}
\def \hatd{\hat{\Delta}}
\def \calC{\mathcal{C}}
\def \calL{\mathcal{L}}
\def \calG{\mathcal{G}}
\def \calF{\mathcal{F}}
\def \calW {\mathcal{W}}
\def \d{\{1,\ldots,d\}}
\def \fstar{f^{*}}
\def \sumn{\sum_{i=1}^n}
\def \sumd {\sum_{j=1}^d}
\def \fracn {\frac{1}{n}}
\def \Dhat {\hat{\Delta}}
\def \xij {x_{ij}}
\def \gn {\|g\|_n}
\def \g2 {\|g\|_2}
\def \gaussg {\left|\fracn \sumn w_i g(\xij)\right|}
\def \rstar {r_n^{*}}
\def \rdstar {r_n^{**}}
\def \rtstar {r_n^{***}}
\def \copt {c_{\mathrm{opt}}}
\def \cone {\theta_1}
\def \ctwo {\theta_2}
\def \cthree {\theta_3}
\def \deltahat {\widehat{\Delta}}
\def \bd {b(d,n)}
\def \bz {\mathbf{z}}
\def \bZ {\mathbf{Z}}
\def \bw {\mathbf{w}}
\def \bW {\mathbf{W}}





\def \sumn{\sum_{i=1}^n}
\def \V{\mathbb{V}}
\def \ihat {\hat{I}}
\def \ihatk {\ihat(k_0,k_*)}
\def \Ik {I(k_0,k_*)}
\def \k0 {k_0}
\def \kstar {k_*}
\def \k1 {k_1}
\def \k2 {k_2}
\def \k3 {k_3}
\def \jhat {\hat{j}}
\def \Pf {\mathbb{P}_f}
\def \Ef {\mathbb{E}_f}
\def \psilk {\psi_{l,k}}
\def \psilprimek {\psi_{l^{'},k}}
\def \alphalk {\alpha_{l,k}}
\def \alphalprimek {\alpha_{l^{'},k}}
\def \bphi {\boldsymbol{\phi}}
\def \bpsi {\boldsymbol{\psi}}
\def \phik {\phi_k}
\def \bphik {\boldsymbol{\phi}_k}
\def \bpsilk {\boldsymbol{\psi}_{l,k}}
\def \sumlk {\sum_{l=1}^{k}}
\def \sumlprimek {\sum_{l^{'}}^{k}}
\def \sumllprime {\sum_{l \neq l^{'}}}
\def \psimax {\|\psi_0\|_{\infty}}
\def \lprime {l^{'}}
\def \jprime {j^{'}}
\def \fmax {\|f\|_{\infty}}
\def \const {C_{\psi_0}}
\def \constf {C(\psi_0,\fmax)}
\def \sumin {\sum_{i=1}^n}
\def \sumjn {\sum_{j=1}^n}
\def \sumij {\sum_{i \neq j}}
\def \sumijs {\sum_{i \neq j\neq s}}
\def \Ei {\mathbb{E}_{f_{X_i}}}
\def \Ej {\mathbb{E}_{f_{X_j}}}
\def \Eis {\mathbb{E}_{f_{X_i},f_{X_s}}}
\def \Ejs {\mathbb{E}_{f_{X_j},f_{X_s}}}
\def \Eij {\mathbb{E}_{f_{X_i},f_{X_j}}}
\def \n2 {\frac{1}{n(n-1)}}
\def \diag {\chi_{n,m} \times \chi_{n,m}}
\def \diagthree {\chi_{n,m} \times \chi_{n,m}\times 
	\chi_{n,m}}
\def \unionm {\bigcup_{m=1}^{M_n}}
\def \pnm {p_{n,m}}
\def \chinm {\chi_{n,m}}
\def \xij {(X_i,X_j)}
\def \xijs {(X_i,X_j,X_s)}
\def \In {\mathbf{I}_n}
\def \vmone {V_{n,m}^{(1)}}
\def \vmtwo {V_{n,m}^{(2)}}
\def \vmone {V_{n,m}^{(1)}}
\def \vmthree {V_{n,m}^{(3)}}
\def \vmcond {\Ef(V_{n,m}|\In)}
\def \summ {\sum_{m=1}^{M_n}}
\def \khat {\hat{k}}
\def \Nm {N_{n,m}}
\def \fmin {f_{\mathrm{min}}}
\def\multint{\int\!\!\cdots\!\!\int}
\def\dint{\int\!\!\int}
\def \bv {\omega}
\def\aa{\check a}
\def\bb{\check b}
\def\AA{\check A}
\let\tilde\widetilde
\let\doubletilde\widetilde
\def\ep{\GG}
\def\epP{\PP}
\def\BV{{\rm BV}}
\def\id{\mathord{\rm id}}
\def\J{{\cal J}}
\def\dsum{\mathop{\mathchar"1350\mathchar"1350}\limits}
\def\ksum{\mathop{\mathchar"1350\mathchar"1350\cdots\mathchar"1350}\limits}
\def\dtilde{\mathaccent"7016}
\def\range{\mathop{\rm Range}\nolimits}
\def \da {\delta a}
\def \db {\delta b}
\def \abg {\aa \bb g}
\def \dg  {\delta g}
\def \gerr {(\delta g +1)}
\def \proja {\hat{\Pi}(\da|\hat{L}^{(k_1,k_2]})}
\def \projb {\hat{\Pi}(\db|\hat{L}^{(l_1,l_2]})}
\def \hg {\hat{g}}
\def \ab {\aa \bb}
\def \projk {\hat{\Pi}^{(k_1,k_2]}}
\def \projl {\hat{\Pi}^{(l_1,l_2]}}
\def \nthree {\frac{1}{n(n-1)(n-2)}}
\def \ktilde {\tilde{K}}
\def \besovb{B_{2,\infty}^{\beta}}
\def \besov {B_{2,\infty}}
\def \mbesov {\mathcal{B}_{2,\infty}}
\def \besovbone{B_{2,\infty}^{\beta_1}}
\def \besovbtwo{B_{2,\infty}^{\beta_2}}
\def \psijkv {\psi_{jk}^v}
\def \constant {C(B,B_U,S)}
\def \bW {\mathbf{O}}
\def \bw {\mathbf{o}}
\def \sumk {\sum\limits_{k \in \Z_j}}
\def \sumv {\sum\limits_{v\in \{0,1\}^d}}
\def \betamin {\beta_{\mathrm{min}}}
\def \betamax {\beta_{\mathrm{max}}}
\def \jmin {j_{\mathrm{min}}}
\def \jmax {j_{\mathrm{max}}}
\def \fhatj {\hat{f}_j}
\def \ghat {\hat{g}}
\def \jstar {j^{*}}
\def \fracg {\frac{g}{\hat{g}}}
\def \deltahat {\hat{\Delta}}
\def \delf {\fhat_n-f}


\def\red{\color{black}}
\def\blue{\color{black}}
\def\green{\color{green}}

\def\itemi{\item{(i)}}
\def\itemii{\item{(ii)}}
\def\itemiii{\item{(iii)}}
\def\itemiv{\item{(iv)}}
\def\itemv{\item{(v)}}
\def\itemvi{\item{(vi)}}


% Abbreviations
\def\A{{\cal A}} \def\a{{\alpha}}
\def\B{{\cal B}} \def\b{{\beta}}                        \def\BB{\mathbb{B}} \def\bB{{\bf B}}
\def\C{{\cal C}}                                        \def\CC{\mathbb{C}}
\def\D{{\cal D}} \def\d{{\delta}}     \def\gD{{\Delta}} \def\DD{\mathbb{D}}
                 \def\e{{\varepsilon}}                  \def\EE{\mathbb{E}} \def\bE{{\bf E}}
\def\F{{\cal F}} \def\f{{\phi}}                         \def\FF{\mathbb{F}}
\def\G{{\cal G}} \def\g{{\gamma}}                       \def\GG{\mathbb{G}}                           
\def\H{{\cal H}} \def\h{{\eta}}                         \def\HH{\mathbb{H}} \def\bH{{\bf H}}
\def\I{{\cal I}}                                        \def\II{\mathbb{I}} 
\def\J{{\cal J}}                                        \def\JJ{\mathbb{J}}              
\def\K{{\cal K}} \def\k{{\kappa}}                       \def\KK{\mathbb{K}}                              
\def\L{{\cal L}} \def\l{{\lambda}}    \def\gL{{\Lambda}}\def\LL{\mathbb{L}} \def\bL{{\bf L}}
\def\M{{\cal M}} \def\m{{\mu}}                          \def\MM{\mathbb{M}}
                 \def\n{{\nu}}                          \def\NN{\mathbb{N}}                              
\def\O{{\Omega}} \def\o{{\omega}}
%\def\P{{\cal P}} 
\def\p{{\pi}}                          \def\PP{\mathbb{P}}
\def\Q{{\cal Q}} \def\q{{\theta}}                       \def\QQ{\mathbb{Q}}
\def\R{{\cal R}} \def\r{{\rho}}				\def\RR{\mathbb{R}}
                 \def\s{{\sigma}}     \def\S{{\Sigma}}  \def\SS{\mathbb{S}}
                 \def\t{{\tau}}       \def\T{{\Theta}}
\def\U{{\cal U}}					\def\UU{\mathbb{U}}
							\def\VV{\mathbb{V}}
\def\W{{\cal W}}                                        \def\WW{\mathbb{W}}
\def\X{{\cal X}} \def\x{{\xi}}				\def\XX{\mathbb{X}} \def\bX{{\bf X}}
\def\Y{{\cal Y}}					\def\YY{\mathbb{Y}} \def\bY{{\bf Y}}
\def\Z{{\cal Z}} \def\z{{\zeta}}                        \def\ZZ{\mathbb{Z}}


\def\sumin{{\sum_{i=1}^n}}
\def\sumjn{{\sum_{j=1}^n}}
\def\sumim{{\sum_{i=1}^m}}
\def\sumjm{{\sum_{j=1}^m}}
\def\sumik{{\sum_{i=1}^k}}
\def\sumjk{{\sum_{j=1}^k}}
\def\tsum{{\textstyle\sum\limits}}
\def\prodjn{{\prod_{j=1}^n}}
\def\prodin{{\prod_{i=1}^n}}
\def\prodim{{\prod_{i=1}^m}}
\def\prodjm{{\prod_{j=1}^m}}
\def\prodik{{\prod_{i=1}^k}}
\def\tprodik{\textstyle\prod_{i=1}^k\limits}
\def\tprod{{\textstyle\prod\limits}}
\def\prodm{\otimes} 
\def\prodmjn{{\bigotimes_{j=1}^n}}
\def\prodmin{{\bigotimes_{i=1}^n}}
\def\tprodmin{{\textstyle\bigotimes_{i=1}^n\limits}}
\def\tprodmjn{{\textstyle\bigotimes_{j=1}^n\limits}}
\def\tprodmim{{\textstyle\bigotimes_{i=1}^m\limits}}
\def\tprodmjm{{\textstyle\bigotimes_{j=1}^m\limits}}
\def\half{{\frac12}}
\def\thalf{{\textstyle\half}}
\def\tkwart{{\textstyle{\frac14}}}
\def\tint{{\textstyle\int\limits}}
\def\tbigcap{{\textstyle\bigcap\limits}}
\def\tbigcup{{\textstyle\bigcup\limits}}
\def\ra{\rightarrow}
\def\da{\downarrow}
\def\ua{\uparrow}
\def\dotfil{\leaders\hbox to 1em{\hss.\hss}\hfill}
\def\minqquad{\hskip-2em\relax}\def\minqqqquad{\hskip-4em\relax}
\def\qqqquad{\hskip4em\relax}\def\qqqqqquad{\hskip6em\relax}
\def\liminfsup{\mathop{\overline{\underline{\rm lim}}}}





% Mathematics
\def\hexnumber#1{\ifcase#1 0\or 1\or 2\or 3\or 4\or 5\or 6\or 7\or 8\or 9\or A\or B\or C\or D\or E\or F\fi}
%\mathchardef\boxminus="3\hexnumber\msafam0C
%\mathchardef\lesssim="3\hexnumber\msafam2E
%\mathchardef\gtrsim="3\hexnumber\msafam26
%\mathchardef\rightsquigarrow="3\hexnumber\msafam20
\def\mypartial#1{\mathchoice{\partial\over\partial#1}{\partial/\partial#1}{}{}}
\def\Re{\mathop{\rm Re}\nolimits}
\def\Im{\mathop{\rm Im}\nolimits}
\def\entier#1{\lfloor#1\rfloor}
\def\BL{{\rm B\kern -0.5pt L}}
\def\UC{{\rm U\kern-0.5pt C}}
\def\linfty{\ell^\infty}
\def\simplex{{\rm S}}
\def\id{id}
\def\argmax{\mathop{\rm argmax}}
\def\argmin{\mathop{\rm argmin}}
\def\trace{{\rm trace }}
\def\diag{\mathop{\rm diag\,}\nolimits}
\def\lin{\mathop{\rm lin\,}\nolimits}
\def\closedlin{\overline{\lin}}
\def\tanh{\mathop{\rm tanh}\nolimits}
\def\arctanh{\mathop{\rm arctanh}\nolimits}
\def\arctg{\mathop{\rm arctg}\nolimits}
\def\loglog{\mathop{\rm loglog}\nolimits}
\def\sign{\mathop{\rm sign}\nolimits}
%\def\interior{{\rm int}}
\def\interior{\mathaccent 23}
\def\closure#1{\overline{#1}}
\def\boundary{\mathop{\delta}\nolimits}
\def\closedhull{{\overline{\hull}}}
\def\closedconv{\closedhull}
\def\essinf{\mathop{\rm essinf}\limits}
\def\conv{\hull}
\def\hull{\mathop{\rm conv\ }\nolimits}
\def\diam{\mathop{\rm diam}\nolimits}
\def\ball{\mathop{\rm ball}\nolimits}
\def\closedball{\overline{\ball}}
\def\every{\hbox{ every }}
\def\forevery{\hbox{ for every }}
\def\OR{\hbox{ or }}
\def\implies{\hbox{ $\Rightarrow$ }}
\def\seilpmi{\hbox{ $\Leftarrow$ }}
\def\bydef{\buildrel {\rm def}\over =}
\def\qed{\ \vrule height4pt width4pt depth0pt}
\def\halmos{\ \vbox{\hrule\hbox{\vrule\vbox{\phantom{\vrule height4pt width4pt depth0pt}}\vrule}\hrule}}

% Statistics
\def\Prodint{\mathop{\mathchoice{\vcenter{\epsfysize=1.5em\epsfbox{%
  prodint.eps}}}{\vcenter{\epsfysize=1em\epsfbox{prodint.eps}}}{}{}}}
\def\prodint{\Prodint}
\def\tdot#1{\kern1.2pt\dot{\vphantom{#1}}\kern-1.2pt
        \dot#1\kern0.8pt\dot{\vphantom{#1}}\kern-0.8pt}
\def\contiguous{\triangleleft}
\def\doublecontiguous{\mathrel{\triangleleft\,\joinrel\triangleright}}
%\def\E{\mathord{\rm E}}
\def\Pr{\mathord{\rm P}}
\def\var{\mathop{\rm var}\nolimits}
\def\sdev{\mathop{\rm sd}\nolimits}
\def\cov{\mathop{\rm cov}\nolimits}
\def\Cov{\mathop{\rm Cov}\nolimits}
\def\cor{\mathop{\rm cor}\nolimits}
\def\Cor{\mathop{\rm Cor}\nolimits}
\let\covar\cov
\let\Covar\Cov
\let\Var=\var
\def\med{\mathop{\rm med}\nolimits}
\def\medlimits{\mathop{\rm med}\limits}
\def\almostsurely{{\rm a.s.}}
\def\almosteverywhere{{\rm a.e.}}
\def\infinitelyoften{{\rm i.o.}}
\def\ae{\almosteverywhere}
\def\ldot{\hbox {$\dot \ell$}}
\def\ltil{\hbox{$\tilde \ell$}}
\def\dirac{\delta}
\def\haslaw{\sim}
\def\haslawunder#1{\mathchoice{\buildrel #1\over \sim}{\ \mathrel{^{#1}}\joinrel\sim}{}{}}
\def\generatedby{\s}
\mathchardef\given="626A
\mathcode`:="603A
%\mathchardef\setminus="2200


% Convergence symbols
\def\generalweak#1{\ {\mathchoice{\buildrel #1\over \rightsquigarrow}%
{\raise-2pt\hbox{$\buildrel #1\over \rightsquigarrow$}}{}{}}\ }
\let\weak\rightsquigarrow
\def\generalprob#1{\ {\mathchoice{\raise-1.5pt\hbox{$\buildrel#1\over\ra$}}
{\raise-2pt\hbox{$\buildrel#1\over\ra$}}{}{}}\ }
\def\outerp{\generalprob {\small P*}}
\def\prob{\generalprob{\small P}}
\def\outeras{\generalprob{\small as*}}
\def\as{\generalprob{\small as}}
\def\vague{\generalprob{\small v}}
\def\au{\generalprob{\small au}}
\def\Pgg{\ {\mathchoice{\raise-1.5pt\hbox{$\buildrel {\small P}\over\gg$}}
{\raise-2pt\hbox{$\buildrel {\small P}\over\gg$}}{}{}}\ }

% Miscellaneous
\def\beginskip{\begingroup\long\def\eet##1\endskip{\endgroup}\eet}
\def\endskip{}
\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern1pt\vbox{\kern1pt #1\kern1pt}\kern1pt\vrule}\hrule}}
\def\eet#1{}
\def\makenumbersactive{\catcode`\0=11\catcode`\1=11\catcode`\2=11%
        \catcode`\3=11\catcode`\4=11\catcode`\5=11%
        \catcode`\6=11\catcode`\7=11\catcode`\8=11\catcode`\9=11 }



\catcode`\@=12







